The Perspective of Software Professionals on Algorithmic Racism

Context. Algorithmic racism is the term used to describe the behavior of technological solutions that constrains users based on their ethnicity. Lately, various data-driven software systems have been reported to discriminate against Black people, either for the use of biased data sets or due to the prejudice propagated by software professionals in their code. As a result, Black people are experiencing disadvantages in accessing technology-based services, such as housing, banking, and law enforcement. Goal. This study aims to explore algorithmic racism from the perspective of software professionals. Method. A survey questionnaire was applied to explore the understanding of software practitioners on algorithmic racism, and data analysis was conducted using descriptive statistics and coding techniques. Results. We obtained answers from a sample of 73 software professionals discussing their understanding and perspectives on algorithmic racism in software development. Our results demonstrate that the effects of algorithmic racism are well-known among practitioners. However, there is no consensus on how the problem can be effectively addressed in software engineering. In this paper, some solutions to the problem are proposed based on the professionals' narratives. Conclusion. Combining technical and social strategies, including training on structural racism for software professionals, is the most promising way to address the algorithmic racism problem and its effects on the software solutions delivered to our society.

==> tables/Questionscomplete.tex <==

%\caption{Survey Questionnaire}
%\label{tab:questinnaire}
%\begin{tabularx}{\linewidth}{p{4cm} p{3.5cm} X}


%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Survey Questionnaire}
\label{tab:questionnaire}
\scriptsize
\begin{tabularx}{\linewidth}{p{5.2cm} p{3cm} X}
Questions &Closed/Open Answer \\\midrule
1. What best describes your gender? &( ) Female \\
&( ) Male \\
&( ) Non-binary \\
&( ) Prefer not to answer \\

2. What best describes your ethnicity? & \\
& \\

3. What diversity group do you identify with (if any) &( ) LGBTQIA+ \\
&( ) Neurodivergence \\
&( ) PWD \\
&( ) Senior (50+) \\
&( ) Prefer not to answer \\

4. Who shares your household with you? & \\
& \\

5. How many years of experience do you have? & \\
& \\

6. How many years have you been working in this company? & \\
& \\

7. What is your primary role in the team? & ( ) Software Design \\
&( ) Software Programming \\
&( ) Software QA \\
&( ) Other role \\

8. Describe an ordinary work week for you. & \\

9. How often are you going to the office lately? &( ) I do not go to the office \\
&( ) Once or twice a month \\
&( ) Once a week \\
&( ) 2 or 3 times a week \\
&( ) 4 or 5 times a week \\
& \\
& \\

10. Main reasons that brought you to the office. 
&( ) I missed the office \\
&( ) I needed a better workspace \\
&( ) I needed technical support \\
&( ) I needed to get away from remote \\
&( ) I wanted to socialize with others \\
&( ) I joined an event \\
&( ) The project demanded \\
&( ) The team needed \\

11. Think about a week that you worked mostly from home. What was good and bad that week? & \\
& \\

12. Think about a week that you worked mostly at the office. What was good and bad that week? & \\
& \\

13. How is your productivity nowadays? &( ) Much higher \\
&( ) Slightly higher \\
&( ) Same as before \\
&( ) Slightly lower \\
&( ) Much lower \\
& \\
& \\

14. Do you usually have to work overtime? &( ) I do not work overtime \\
&( ) Up to 2 hours/week \\
&( ) 2 to 5 hours/week \\
&( ) More than 5 hours/week \\
& \\

15. What is the best hybrid work arrangement? &( ) Mostly remote \\
&( ) Voluntarily going to the office \\
&( ) Weekly pre-defined days at the office \\
&( ) Monthly pre-scheduled days at the office \\
&( ) Mostly at the office \\
\bottomrule
\end{tabularx}
\end{table}

==> tables/benefits.tex <==

%\caption{Survey Questionnaire}
%\label{tab:questinnaire}
%\begin{tabularx}{\linewidth}{p{4cm} p{3.5cm} X}


%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Benefits of Refactoring in Testing Code}
\label{tab:benefits}
\scriptsize
\begin{tabularx}{\linewidth}{p{1cm} p{5cm} p{2cm}}
%\begin{tabular}{ccc}
  &  & \% of Participants \\\midrule

 & Support automation code maintenance & 75\% \\
 & Improvement of code readability & 60\% \\
 & Increase of automation reusability & 56\% \\
 Benefits & Removal of duplicated code & 41\% \\
 & Improvement of test automation performance  & 35\% \\
 & Improvement of team performance & 26\% \\
 & No observable benefit & 4\% \\
%\end{tabular}
\bottomrule
\end{tabularx}
\end{table}


 







==> tables/limit.tex <==

%\caption{Survey Questionnaire}
%\label{tab:questinnaire}
%\begin{tabularx}{\linewidth}{p{4cm} p{3.5cm} X}


%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Challenges of Refactoring in Testing Code}
\label{tab:limit}
\scriptsize
\begin{tabularx}{\linewidth}{p{1cm} p{5cm} p{2cm}}
%\begin{tabular}{ccc}
  &  & \% of Participants \\\midrule

 & Time-consuming & 79\% \\
 & No interest from managers/leaders & 59\% \\
 & Lack of knowledge on refactoring & 51\% \\
Challenges & Complexity of changes & 20\% \\
 & Changing test code that is working & 19\% \\
 & Tools unavailability & 16\% \\
 & No significant gain & 15\% \\
 & Lack of priority & 2\% \\
%\end{tabular}
\bottomrule
\end{tabularx}
\end{table}


 









 







==> tables/types.tex <==

%\caption{Survey Questionnaire}
%\label{tab:questinnaire}
%\begin{tabularx}{\linewidth}{p{4cm} p{3.5cm} X}


%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Types of Refactoring in Testing Code}
\label{tab:types}
\scriptsize
\begin{tabularx}{\linewidth}{p{2cm} p{4cm} p{2cm}}
%\begin{tabular}{ccc}
  &  & \% of Participants \\\midrule

 & Changing the structure of methods & 76\% \\
 & I needed a better workspace & 75\% \\
Refactoring Types & I needed technical support  & 50\% \\
 & I needed to get away from remote & 49\% \\
 & I wanted to socialize with others & 5\% \\
%\end{tabular}
\bottomrule
\end{tabularx}
\end{table}
